Do LLMs Speak the User's Language? A Study of Personalized Language Selection in Multilingual LLMs

Large Language Models increasingly interact with multilingual users, yet personalization of LLMs' response-languages remains overlooked. We present the first systematic study of user-aware response-language generation: customizing response-languages to users' linguistic background inferred from prior interactions. To this end, we introduce PULSE, a benchmark of code-switched dialogue histories, queries, and user-conditioned reference responses, with linguistically grounded automated evaluation. Experiments reveal that LLMs are driven by surface cues in the query, often responding in a user-inappropriate form. To mitigate this challenge, we propose a two-stage alignment pipeline, comprised of supervised grounding on dialogue-derived user cues and reinforcement-learning post-training with user-aware rewards. Our dataset and code are released at https://github.com/LaMI-Labs/PULSE.

==> manuscript/Check.tex <==
% --------------------------------
% Introduction 
% --------------------------------
\section{Introduction}

Large language models (LLMs) are increasingly deployed as conversational assistants across a wide range of real-world applications, making it important to understand how effectively they support human users~\cite{ou2024dialogbench, zhao2025personalens}. 
% --------------------------------

Despite the expanding scope of LLMs' applications, existing evaluations and benchmarking of LLMs have largely focused on task accuracy, reasoning ability, and problem-solving performance in isolated question-answering settings~\cite{hendrycks2020measuring,cobbe2021training,srivastava2023beyond}. 
% --------------------------------


When LLMs engage in sustained interaction with humans, however, additional challenges emerge that are not readily captured by such single-turn evaluations. 
In particular, failure to retain user-relevant information or remain consistent with prior interactions can substantially undermine users' engagement~\cite{cox2023comparing,maharana2024evaluating,tan2025prospect} and trust~\cite{baughan2023mixed,landerberg2026trust} in future interactions.
% --------------------------------


Consequently, personalization, the ability to adapt model behavior and responses to the characteristics, preferences, and needs of individual users, has become an increasingly important research direction for improving the quality of user experience and overall satisfaction~\cite{chen2024recent,westhausser2025enabling}.

% --------------------------------


Prior works on personalization have primarily focused on customizing the \textit{content} of the model response on users' personal characteristics, interests, preferences, or interaction histories~\cite{cheng2024dialogues,liu2025llms+}. 

% --------------------------------

In contrast, the question of \textit{in what linguistic form} that content should be delivered in a user-tailored manner has received relatively limited attention~\cite{blevins2026language}.
For instance, a multilingual user may prefer general explanations in their native language while being more familiar with technical terminology in English, making a carefully code-switched response more natural and comprehensible than a fully monolingual one~\cite{brixey2026can}.
% --------------------------------


In this work, we study~\textit{user-aware response-language generation}, the task of selecting and combining languages in a response based on an individual user's linguistic background and prior interactions.
Successfully carrying out this task enables LLMs to adapt their response-language to individual users, supporting more natural and socially appropriate interactions while conveying language-specific knowledge and cultural nuances more effectively.


User-aware response-language generation differs from conventional content personalization in two important respects. 
First, the model must infer the user’s linguistic background and proficiency from their prior interactions. 
This inference is non-trivial because such attributes are rarely stated explicitly and must instead be recovered from indirect signals in the dialogue history~\cite{mok2025exploring}. In our setting, these signals include language choice, lexical usage, and code-switching patterns. 

% --------------------------------

Second, the LLMs must turn this understanding into the most appropriate response-language while preserving semantic fidelity, fluency, and discourse coherence.
This user-aware response-language selection process is further complicated by the limited ability of current LLMs to produce natural and contextually appropriate code-switched text~\cite{kuwanto2026linguistics}. 
% --------------------------------

\begin{figure*}[t]

  \includegraphics[width=\textwidth]{figure/fig1_sh_v5.pdf}
  \caption {Illustration of user-aware response-language generation. Given the same Korean--English code-switched query, the query-focused response follows the surface form of the query, whereas the user-aware response adapts the language of the explanation to the user's Korean proficiency inferred from prior dialogue while preserving the culture-specific term \textit{imo} (`auntie').}
  \label{fig1:example}
  \vspace{-10pt}
\end{figure*}

To systematically investigate aforementioned challenges, we introduce~\textbf{\ourdata}~(\textbf{P}ersonalized \textbf{U}ser-aware \textbf{L}anguage \textbf{S}election \textbf{E}valuation), a new diagnostic dataset and evaluation framework for user-aware response-language generation. 
We construct~\ourdata~by synthetically generating multi-turn, code-switched dialogue histories that implicitly reveal a user’s linguistic background and proficiency. 
Each dialogue history is paired with a code-switched query and a ground-truth target response whose linguistic form is conditioned on the user information conveyed in the preceding interactions. 
By presenting the same query under different user profiles, this design enables us to isolate whether models adapt their response-language to information revealed through dialogue history rather than merely following the linguistic form of the query. 
Further details of the dataset construction process are provided in Section~\ref{sec3:pulse}.

Our initial exploration with~\ourdata~reveals that current LLMs do not reliably adapt their response-language choices to users’ linguistic backgrounds. 
Instead, their response-language is heavily influenced by the surface-level linguistic structure of the final query. 
As illustrated in~\figurename~\ref{fig1:example}, a code-switched query does not necessarily reveal which the user's proficiency in each language or their preferred language for extended explanations. 
Nonetheless, model responses remain strongly anchored to the linguistic patterns of the query, even when relevant dialogue history or structured user information is provided. 
This finding highlights a key blindside of query-centered approaches to response-language selection~\cite{oh2026ola}; meaningful personalization requires LLMs to look beyond the most recent utterance and draw on interaction history to infer user-specific linguistic characteristics and preferences.

\jm{To mitigate this limitation, we perform supervised fine-tuning (SFT) using dialogue--query--response instances. 
This trains the model to directly generate responses that reflect user information revealed in prior dialogue. 
We analyze the generated responses using a Korean--English matrix-language classifier that incorporates syntactic information, and compare the distribution of response forms across user profiles and query types. 
Our experimental results show that targeted SFT elicits user-appropriate response forms more consistently than prompting-based approaches. 
This finding highlights the need for targeted alignment training for user-aware response-language generation.}

Our contributions are as follows:
\begin{itemize}
\item We formulate the problem of user-aware response-language generation in code-switched interaction, where the appropriate monolingual or mixed-language response form depends not only on query-level linguistic cues but also on the user’s implicit linguistic background, proficiency, and language-use patterns.

\item We introduce ~\ourdata~, a diagnostic dataset and evaluation framework that combines OLA-based queries, newly constructed culture-based Korean--English code-switched queries derived from Korean cultural data, proficiency-conditioned synthetic dialogues, and user-appropriate target responses.

\item We show that prompting alone does not reliably induce user-aware response-language adaptation. Through a distributional analysis of response forms using a syntax-aware matrix-language classifier, we further demonstrate that targeted SFT improves the generation of language forms appropriate for individual users.

\end{itemize}


% --------------------------------
% --------------------------------
% --------------------------------
% --------------------------------

\section{Related Work}

\subsection{Personalization of LLMs}
\label{relate2.1}
Personalization, the process of tailoring LLMs' responses to individual users, plays a crucial role in the user experience of LLM-based conversational systems~\citep{tseng2024two}. 
Although personalization has become increasingly important, even frontier LLMs often fail to tailor their responses appropriately to individual users~\citep{jiang2025know}.
Early works in personalization aimed to condition the generation process on persona statements or user-specific records that were directly available in the context~\citep{zhang2018personalizing, salemi2024lamp}.
Recent works have begun to explore more realistic and practical scenarios in which the model must infer them from its previous interactions with the user~\citep{zhao2025llms, zhong2025evaluating}.
Similarly, our work explores whether LLMs can adapt their responses to a user's linguistic background, which can be inferred from previous dialogue turns.

To the best of our knowledge, our work is the first to extend personalization beyond the~\emph{content} of a response to its~\emph{linguistic form}, adapting how LLMs' responses are styled to the user’s background. 
Most closely related to our work,~\citet{xu2026controlling} customize the linguistic difficulty of responses to the proficiency of second-language learners. 
Their approach, however, modulates complexity within a single, predetermined target language rather than selecting or combining languages according to the user’s linguistic background.

% --------------------------------
% poplack2013sometimes 수정(Researchgate 버전) 
\subsection{Code-Switching and Response-Language Generation}
Code-switching (CS), the alternation between two or more languages within an utterance or discourse, is a natural communicative practice among multilingual speakers~\citep{poplack2013sometimes}.

Early code-switching research focused primarily on natural language understanding, evaluating language models' ability to process code-switched input input~\citep{khanuja2020gluecos,winata2021multilingual,prasad2021effectiveness}.

Moving beyond these understanding-focused evaluations, recent studies have begun to examine whether LLMs can generate fluent and linguistically plausible code-switched text~\citep{yong2023prompting,kuwanto2026linguistics}.

However, these generation studies primarily evaluate models' general code-switching generation capabilities and the linguistic quality of their outputs, without addressing which linguistic form is appropriate in a particular interaction.

\citet{oh2026ola} evaluate whether LLMs can infer the implicitly expected output language from cues in the current query.
However, this query-centered formulation does not account for the possibility that the same query may warrant different response forms for different users.

Our work therefore extends query-centered output-language alignment to user-aware response generation and evaluates whether LLMs can generate an appropriate monolingual or code-switched response according to each user's language proficiency.

% --------------------------------
% --------------------------------
% --------------------------------
% --------------------------------
